Design, Development and Experimental Realization of a Quadrupedal Research Platform: Stoch

In this paper, we present a complete description of the hardware design and control architecture of our custom built quadruped robot, called the `Stoch'. Our goal is to realize a robust, modular, and a reliable quadrupedal platform, using which various locomotion behaviors are explored. This platform enables us to explore different research problems in legged locomotion, which use both traditional and learning based techniques. We discuss the merits and limitations of the platform in terms of exploitation of available behaviours, fast rapid prototyping, reproduction and repair. Towards the end, we will demonstrate trotting, bounding behaviors, and preliminary results in turning. In addition, we will also show various gait transitions i.e., trot-to-turn and trot-to-bound behaviors.

==> Making.tex <==
\section{Materials and Manufacturing}\label{sec:making}

In this section, we will discuss 
1. material selection to keep robot leg and body lightweight
2. designing for rapid prototyping(3d printing) and 
 

\subsection{Definitions}

==> Unlisted.tex <==


\section{Reinforcement Learning Framework for Quadrupedal Walking}\label{sec:rl}

In this section, we will study the deep reinforcement learning (D-RL) framework used for realizing quadrupedal walking in simulation. We will also discuss the associated challenges with the learning methods, and the transferability issue from simulation to real hardware.

\subsection{Definitions}
We formulate the problem of locomotion as a Markov Decision Process (MDP). An MDP is represented by a tuple $\{S, A, P, R, \gamma \}$. Here $S \in \R^n$ is the set of robot states referred to as state space, and $A \in \mathbb{R}^m$ is the set of feasible actions referred to as the action space. $P: S\times A \times S\rightarrow [0,1]$ is the transition probability function that models the evolution of states based on actions, and $R: S \times A \rightarrow \R$ is the reinforcement or the reward obtained for the given state and action. $\gamma$ is called the discount factor defined in the range $[0,1]$. 

The goal in RL is to achieve a policy that maximizes the expected cumulative reward over time. A policy, denoted as $\pi: S \times A \to [0,1]$, is the probability distribution of the actions over the states. When dealing with huge state and action spaces, a parametrized policy is used, denoted as $\pi_\theta$, with the parameters $\theta$. The optimal parameters and/or policy yields the maximum sum of the cumulative rewards. %Since the policy is a distribution, 
We use the following to obtain the optimal policy $\pi_{\theta^*}$: 
\begin{align}
\theta^* = \arg \max_\theta \sum\limits_{t=1}^{T} \E_{(s_t, a_t) \sim p_{\pi_\theta}(s_t, a_t)}[R(s_t, a_t)],
\end{align}
where $p_{\pi_\theta}$ is the marginalization of the state-action pair given the set of all possible trajectories $(s_0, a_0, s_1, a_1, ..., s_T)$ following policy $\pi_\theta$. The optimal parameters $\theta^*$ are evaluated iteratively by taking gradient ascent steps in the direction of increasing cumulative reward. More details on the algorithm, and the associated optimization technique are provided in Section \ref{algo}.

%The particular choice of action space can be easily bounded for the hardware safety, covers all permitted leg configurations and most importantly reduce the training time and improve the efficiency.
% \begin{figure}[h!]
% \includegraphics[width=\linewidth]{learning_arch1.jpg}
% \label{fig:training_loop}
% \caption{Reinforcement learning training framework}
% \end{figure}



\subsection{State and Action Space}

\label{sec:model}
%\section{Hardware Description}
We will briefly describe the quadrupedal model of Stoch.  
% All the four legs of the robot are identical and arranged in a symmetric fashion. 
There are four identical legs and eight actuators in the robot which are distributed equally among its joints. Each leg has a hip and a knee joint, and the actuators provide flexion-extension in each joint. Fig. \ref{fig:robot_pic} shows both the experimental and the simulated robot model.
% Each leg is identical, and has a total of 2 degrees of freedom: hip flexion-extension and knee flexion-extension. Hence, there are totally eight actuators in Stoch. 
Details on the experimental model are in Section \ref{sec:results}.

\subsubsection{State Space}
The state for the training is represented by angles, velocities and torques of the active joints. Body orientation (in quaternions) is also included in the state space. The combined representation yields a 28D state space. 
Note that the motor torques are typically treated as states in RL framework.
% This is a deviation from the traditional (control theoretic) definition of state space.
% (cite the google paper and the equation number where they included torque in the statespace).
% However, calculating velocities and accelerations is noisy on a physical system, therefore we are using joint-angles and base orientation (in quaternions) as the state space in our problem. 
\subsubsection{Action Space}
Reference \cite{action_space} demonstrated the effectiveness of choosing actuator joint angles as action space. The planar four bar linkage configuration of the legs, however, lead to self-colliding regions in the motor space. This creates a non-convex search space and degrades the learning efficiency. Hence, we chose to learn the legs' end-point position in polar coordinates represented as $\{r_i, \alpha_i\}$ where $i \in \{1,2,3,4\}$. The polar coordinates for the four legs collectively provide an $8$ dimensional action space. For each $r_i, \alpha_i$, we can obtain the joint angles (both hip and knee of leg $i$) via an inverse kinematics solver. We will denote the angles obtained from the inverse kinematics solver as $\{\beta_i^1, \beta_i^2\}$. % for each leg subjecting to the constraints to avoid internal collisions.   
% The learned end-point positions are fed into an inverse kinematic solver that provides the motor angles $\{\theta_i^1, \theta_i^2\}$ for each leg, to be executed by the robot. 
The polar coordinates can be restricted to a bounding box, thereby indirectly imposing angle limits on the joint angles.

\subsection{Network and Learning Algorithm} \label{algo}
Since the states and actions are continuous, we seek for algorithms that enable us to construct optimal policies that yield action values in the continuous space. Proximal Policy Optimization (PPO) \cite{PPO} have proved to be very successful for obtaining optimal continuous action values \cite{rlmatters}. It is an on-policy, model-free algorithm based on actor-critic learning framework. An actor (also called policy) decides an action given a state and a critic aims to improve the policy by evaluating the action value function. Both actor and critic networks are parameterized by neural networks with parameter $\theta$ and $\phi$ respectively. 
% 	Both of these neural networks consist of two fully connected layers with the first and second layers consisting of 200 and 100 nodes respectively. Activation units in the actor and critic networks are ReLU $\rightarrow$ ReLU $\rightarrow$ tanh, and ReLU $\rightarrow$ ReLU $\rightarrow$ linear respectively.

The learning algorithm samples $N$ episodes of maximum length $T = 1000$ using the current policy. The experience tuples consisting of $\{s_t, a_t, s_{t+1},r_t \}$, with $t \in [0, T]$, are stored and used for on-policy update of the parameters.
Policy gradient method \cite{advantage} gives the objective function to optimize the policy parameters given as:
% To optimize the policy parameters Sutton et al.\cite{advantage} provided the objective functions as:
\begin{align}
L^{PG}(\theta) = \E_{\pi_\theta} \Big[\log\pi_\theta(a_t|s_t)\hat{A_t}\Big]
\end{align}
where $\hat{A_t}$ is called the estimated Advantage function. It is given by $\hat{A_t} = r(s_t, a_t) + \gamma V_\phi(s_{t+1}) - V_\phi(s_t)$, where $V_\phi$ is the value function at any state. Furthermore, in order to account for the disparity between the behavioral policy $\pi_{old}$, and the current updating policy $\pi_\theta$, the advantage estimation is multiplied with the importance sampling ratio given by
\begin{align}
L(\theta) = \E_{\pi_{old}} \Bigg[\dfrac{\pi_\theta(a_t|s_t)}{\pi_{old}(a_t|s_t)}\hat{A_t}\Bigg].
\label{impotance_sampling}
\end{align}
% Lastly, in order to avoid huge and sudden variations in the policy during training TRPO \cite{TRPO} puts a constraint on the KL-divergence between the old and the new policy. However, the PPO algorithm simplifies the process by penalizing on the high KL-divergence and solving an unconstrained optimization. Hence the final objective for the PPO algorithm is given by
Lastly, in order to avoid huge and sudden policy variations during training, PPO penalizes on the high KL-divergence and solves an unconstrained optimization. Hence the final objective for the PPO algorithm is given by
\begin{align}
\begin{split}
L^{KL}(\theta) = \: &\E_{\pi_{old}} \Bigg[\dfrac{\pi_\theta(a_t|s_t)}{\pi_{old}(a_t|s_t)}\hat{A_t}\Bigg] - \\ & \beta_{KL} \E_{\pi_{old}}\big[ D_{KL} (\pi_{old}(a_t|s_t) || \pi_{\theta}(a_t|s_t)) \big]
\end{split}
\end{align}
where $\beta_{KL}$ is an adaptive penalty coefficient. Given a target KL-divergence $\delta$, $\beta_{KL}$ for next policy update is calculated as:
\begin{itemize}
\item if $D_{KL} < \delta/1.5, \beta_{KL} \leftarrow \beta_{KL}/2 $
\item if $D_{KL} > \delta/1.5, \beta_{KL} \leftarrow \beta_{KL} \times 2 $
\end{itemize}

We used the open source implementation of PPO by Tensorflow Agents \cite{tf_agents} that creates the symbolic representation of the computation graph. The implementation is highly parallelized and performs full-batch gradient ascent updates, using Adam \cite{adam} optimizer, on the batch of data collected from multiple environment instances.


\subsection{Simulation Framework}
We used Pybullet \cite{pybullet} simulator, built on top of Bullet3 physics engine, for a realistic model simulation. A three-dimensional computer-aided-design (CAD) model is developed using SolidWorks \cite{solidworks} to capture the kinematics and inertial properties of the robot. This model is transferred to Pybullet by using a Universal Robot Description Format \cite{roswebsite}
 (URDF) exporter. In addition, actual mass of all the links, actuator force limits, joint limits and kinematic-loop constraints of the flexural joints are measured and manually updated in the URDF file for a more realistic simulation (refer Fig. \ref{fig:robot_pic}). 

\subsection{Reward Function}
We designed a reward function that gives positive reinforcement with the increasing robot's base speed and simultaneously penalizes high energy consumptions. The agent receives a scalar reward after each action step according to the reward function
\begin{align}\label{eq:reward}
r_t = w_{vel} \cdot {\rm{sign}}(\Delta x_t) \cdot \max \{ | \Delta x_t |, 0.1 \} - w_E\cdot \Delta E .%|\tau_t\cdot \omega_t|\cdot \Delta t
\end{align}
Here $\Delta x_t$ is the difference between the current and the previous base position along the $x$-axis. %$\tau$ and $\omega$ are the motor torques and motor velocities respectively. $\Delta t$ is the simulation time step 
$\Delta E$ is the energy spent by the actuators for the current step,
and $w_{vel}$ and $w_E$ are weights corresponding to each term. $\Delta E$ is computed as
\begin{align}
\Delta E = \Sigma_{i=1}^4 ( | \tau^1_i (t) \cdot \omega^1_i (t) | + | \tau^2_i (t) \cdot \omega^2_i (t) | ) \cdot \Delta t,
\end{align}
where $\tau^1_i, \tau^2_i$ are the motor torques, and $\omega^1_i, \omega^2_i$ are the motor velocities of the $i^{th}$ leg respectively.

\subsection{Gait Generation and Simulation Results}
% \subsubsection{Gait Design}
The actor and critic network in the learning algorithm consists of two fully connected layers with the first and second layers consisting of 200 and 100 nodes respectively. Activation units in the actor and critic networks are ReLU $\rightarrow$ ReLU $\rightarrow$ $\tanh$, and ReLU $\rightarrow$ ReLU $\rightarrow$ linear respectively. Other hyper-parameters are mentioned in Table. \ref{tab:hyperparam}. The pybullet simulator is configured to spawn multiple agents for faster collection of samples---in our case 30 agents were used in parallel threads. 



Quadrupedal animals typically have eight types of gaits \cite{owaki2017quadruped,Fukuoka2015}. Work done in \cite{DBLP:journals/corr/abs-1803-05580} used reference trajectories and \cite{google_paper} used open-loop signal to learn a specific gait. However in this work, we learned everything from scratch. To learn a specific gait type, we leveraged gait symmetries and put hard constraints on the foot position. For e.g. in trot, diagonally opposite legs are in sync. Hence, we provide same $\{r, \alpha \}$ to  these legs. This also results in reduction in the dimensions of action space from $8$ to $4$. 
% To learn a specific gait type we put hard constraints on the legs' phase difference (e.g. in trot, diagonally opposite legs have the same phase resulting in reduction in the dimensions of action space from $8$ to $4$). 

The proposed approach yields walking gaits that are efficient, fast and also robust in simulation. The learning algorithm runs for a maximum of $15$ million steps and the observed training time is $4.35$ hours on a Intel Core i7 @3.5Ghz$\times 12$ cores and 32 GB RAM machine.

\begin{table}[t!]
\centering
\begin{tabular}{ c | c }
  Entity & Value  \\
  \hline
  $w_E, w_{vel}$ & $0.05, 1.0$  \\
  Discount factor $(\gamma)$ & $0.994$ \\
  Learning rate (actor, critic) & $10^{-4}, 10^{-4}$ \\
  Training steps per epoch & $3000$  \\
  KL target ($\delta$) & $0.01$  \\
  End-point position limit ($\theta$) & $[\ang{-30},\ang{30}]$\\
  End-point position limit ($r$) & $[15$cm, $24$cm$]$\\
\end{tabular}
\caption{\small Hyper-parameter values of the learning algorithm}
\label{tab:hyperparam}
\end{table}
% For the rest of the paper we will mainly use the trot gait as reference; but the approach has also been successfully used to generate other gaits.

%Using prior knowledge of the gaits, than restructuring the reward function to generate different gaits from scratch, speeds up the learning process. Therefore, we put hard constraints on the legs' phase difference (e.g. in pace, legs on each side have the same phase). This constraint effectively reduce the dimensions of the action space from $8$ to $4$.

\subsection{Challenges}

There are two main challenges in realizing D-RL based gaits in quadrupeds:

\subsubsection{Training for model and environment updates} The training framework has a large set of hyper-parameters (a small subset of them are shown in Table \ref{tab:hyperparam}) that require tuning in order to get desirable gaits. These gaits are, indeed, robust and efficient, but any update in the model or change in constraints in the gait requires retuning of these hyper-parameters in order to obtain desirable gaits. Retuning is not intuitive and requires a series of training iterations.
This is a common problem even in nonlinear model based walking optimizations \cite{reher2016algorithmic}, where small variations in constraints often lead to infeasible solutions.  


\subsubsection{Transferability on real hardware}

Transferability of these learned gaits in the real hardware faces numerous challenges. Some of them are mainly due to uncertainties due to unaccounted compliances, imperfect sensors, and actuator saturations. In addition, inertial and electrical properties of  actuators vary from one joint to another. %These uncertainties often resulted in unrealizable gaits from the training. 
It can be observed that imposing very conservative constraints like tighter velocity and angle limits resulted in longer training times, which often converged to very unrealistic gaits. 

In order to put these challenges in context, it is necessary to review the methodology followed in \cite{google_paper}. They proposed to develop accurate robot model, identify the actuator parameters and study the latencies of the system. This procedure, indeed, resulted in more realistic gaits, but required multiple instances of training and is highly sensitive for any update in hardware. In addition, DNNs are computationally intensive (NVIDIA Jetson TX2 processor was used). Therefore, as a deviation from this approach, we primarily want to focus on a methodology that is more robust to hardware changes, and also computationally less intensive. As we add more and more tasks and objectives for a diverse set of environments, it is important to focus on using a {\it compressed} set of walking parameters with minimal training. 
% We propose a solution that uses kinematic motion primitives (kMPs) extracted from principal component analysis (PCA). 
% We will show that it is possible to reconstruct the walking gaits learned by the DNNs via a minimal set of trajectories, called the kinematic motion primitives (kMPs). 
We will discuss this in detail in the next section. 



%It was shown in \cite{moro2012kinematic} that a set of simple human demonstrations of multiple tasks 



%We not only get realizable behaviors but also can obtain derived behaviors like bounding and walk.

%walking gaits in the quadrupedal robots and the naturally occurring gaits in the animals.


%On the other hand, it is important to note that traditional techniques for realizing efficient and robust walking in legged robots involve extensive comparisons with animal data. 


 %It was observed (refer Fig \textbf{TODO}) that the kinematic motion primitives that describe the basic patterns for the animals have a high correlation with the kMPs of the trajectories obtained from the simulation and hardware.


% Start discussing the simulation results, and also show different cases, examples, scenarios, environments, tuned parameters.


% While PPO yields walking gaits in the simulator that are efficient and robust and also yield animal like walking behaviors, translation of these gaits in the actual systems faces numerous challenges. Some of them are mainly due to uncertainties, wrong modeling frameworks, and imperfect sensing and actuations. On the other hand, it is important to note that traditional techniques for realizing efficient and robust walking in legged robots involve extensive comparisons with animal data. It was shown in ijspeert that basic walking patterns in biological quadrupeds (like horses) inherently contain some components that are consistent across different gaits. With this as the motivation, we considered studying the gaits obtained from the simulators, i.e., comparison between artificially obtained walking gaits in quadrupedal robotos and the naturally occuring gaits in animals. It was observed that the principal components that describe basic patterns for animals have a high correlation with the prinicap components obtaine from the simulation. Show some figure.s







==> temp.tex <==
Section \ref{sec:results/HWexp} describes the results of the implementation of kMP in the hardware. Section \ref{subsubsec: data_compare} shows the comparison of the kMP between the trot gaits learned in robot simulation, implemented in hardware and extracted from horse. Horse kMP was extracted by digitizing the plots from \cite{moro2013horse}. The tables in this section report only the final results of the statistics applied. In section \ref{subsubsec: Gait_change}, we change gait from trot to pace and vice verse by just switching the elements of the weight matrix. In section \ref{subsubsec: Turning}, we generate turning motion by manipulating the weights of the weight matrix.
\subsubsection{Experimental setup}\label{subsubsec: Exp_setup}
The experiments on the hardware is conducted on flat terrain. the details of the test can be seen in these\textbf{VIDEO} videos.
All the tests were conducted at 2.5 Hz frequency.  
\subsubsection{Data comparison}\label{subsubsec: data_compare}


\begin{figure*}[h!]
\centering
\includegraphics[width=\linewidth]{kMP_trot_grd.pdf}
  \caption{kMP for trot}
  \label{fig:kMP_trot}
\end{figure*}


Some of the kMPs, as it can be seen, share some common features with other gaits. To observe if these gaits a have any common kMP we super impose one plot over. Following diagram  shows the superimposed plot.

While analyzing the data, we compared the extracted kMP with some of the kMP of animals found in the literature. A comparison with the horse kMP can be seen in the figure \ref{fig:kMP_BioVsRL}. 
\begin{figure}[h!]
\includegraphics[width=\linewidth]{kMP_HorseVsRL.pdf}
  \caption{Comparison between the horse kMP and the RL learned kMP in trot gait}
  \label{fig:kMP_BioVsRL}
\end{figure}

\begin{table}
\centering
\begin{tabular}{c||c|c|c|c||c|c}
 & 1st & 2nd & 3rd & 4th & Average & Weighted\\
\hline
RLT1-RLT2 & 0.99 & 0.93 & 0.82 & 0.78 & - & -\\
RLT1-HT & 0.951 & 0.979 & 0.936 & 0.656 & - & - \\
RLT2-HT & 0.97 & 0.99 & 0.77 & 0.55 & - & - 
\end{tabular}
\caption{Statistical analysis of similarity among kMPs extracted from Reinforcement learned trot(RLT1 and RLT2) and Horse trot kmp(HT) - cross-covariance}
\end{table}
\begin{table}[h!]
\centering
\begin{tabular}{c||c|c|c|c||c|c}
 & 1st & 2nd & 3rd & 4th & Average & Weighted\\
\hline
RLT1-RLT2 & 0 & -0.02 & -0.09 & -0.01 & - & -\\
RLT1-HT & -0.03 & 0 & 0 & 0.5 & - & - \\
RLT2-HT & 0 & 0.02 & -0.1 & -0.05 & - & -
\end{tabular}
\caption{Statistical analysis of similarity among kMPs extracted from Reinforcement learned trot(RLT1 and RLT2) and Horse trot kmp(HT) - Delay}
\end{table}

==> unlisted_ajay.tex <==
\section{SOFTWARE}
In this section we describe software related concepts developed for the Oncilla robot; namely the communication bus connecting main control boards and periphery, the motor controller, Oncilla robot’s software architecture.

\subsection{Communication Layer and Protocol}
Communication between main electronic modules is performed over a RS-485 physical layer, organized in a master/slave pointto-multipoint half-duplex configuration (Figure 4). The data link and network layer on the bus is implemented through a custom Simple Binary Communication Protocol (SBCP).
Latter implementation is an extension of the Bioloid Dynamixel Communication Protocol version 1 (Robotis Ltd., Co, 2018). The main modification is the change of the two byte packet preamble value 0xFFFF). This preamble was separated; one single byte preamble (0XFF), and a ClassID byte to designate the device type we want to address, i.e., the motor driver board, power board, or master control board. By reserving the class value for Bioloid devices, Oncilla robot’s hardware and driver are capable of directly incorporating these. A major challenge in the SBCP design was the high communication bandwidth requirement. We initially aimed at a 1 kHz control loop on the embedded computer level, this translates to a RS-485 baud rate of 3.3Mbps. Recently such high speed UARTs became available in embedded computers (< 12Mbps at the moment), through an USB to serial Integrated Circuit (IC). However, USB bus communication is scheduled by 1ms frame sizes, and a naive bus implementation would be limited to reach a device every 2ms. Instead, we implemented a bus control data flow in a dedicated device (SBCP master board) controlled by a dsPIC33FJ128MC802 Digital Signal Processor (DSP), mounted after the USB to serial IC. This SBCP master board is able to: 
\begin{itemize}
    \item Handle a group of up to 8 combined packets sent over a full duplex UART connection.
    \item Manage communication over the half duplex RS-485 bus with a latency of 12 μs and maximal jitter of 2.2 μs. 
    \item Detect slave timeouts and react accordingly with user customizable delays.
\end{itemize}

To reduce jitter and latency to a minimum, we utilized many optimization features of the dsPIC33FJ processor
family such as Direct Memory Access (DMA), reduction of interruption stress on the processor, and anticipated packet pre-computation and pre-buffering to reduce latency between packet responses. All implementation details are abstracted by a reusable library, SBCP-uc 4. This new open source library enables fast development of slave device SBCP interfaces for this processor family.

\subsection{Motor Control}
The custom designed motor driver boards implement a Proportional-Integral-Derivative (PID) controller for two
brushless motors on a dsPIC33JF128MC804 DSP. It controls two A3930 motor driver ICs which are used to drive a three phase inverter made of six IRFR48Z MOSFETs. These ICs are able to limit the motor winding current. DSP PID controller parameters were hand tuned. In order to reduce motor jitter during position tracking, a velocity profile interpolation is implemented on the motor driver DSPs. The user sets the desired tracking frequency, and the tracking velocity is then computed on-board. Initially we observed trajectory tracking losses every several seconds. We found the cause in a combination of communication jitter and real-time clock frequency mismatch. Tested RB-110 boards had crystal frequency deviations of up to +0.3 \%, from their standard frequency. As a workaround, we implemented precise buffering and real-time clock re-synchronization heuristics on the motor driver DSP. The maximum tracking frequency is 500Hz, half of the DSP internal control loop (1 kHz).

\subsection{Software Architecture}
The software architecture of Oncilla robot is based on two primary design decisions tied to the requirements of open
research projects (Nordmann et al., 2013): (a) It provides a common interface for the simulator and for the hardware. This allows for easy and fast transition of experiments between simulation and real-world experiments. (b) It provides a local interface for fast control loops running on the embedded PC, as well as a remote interface to allow more complex applications to control the robot over the network. Figure 5 shows the software architecture that exposes the abstracted interface for both simulation and hardware at different application programming
interface (API) levels according to application requirements.

\subsection{Simulation and Robot Interface}
One of the main design goals was to implement a common abstraction between hardware and simulation, with binary compatibility, to facilitate an easy transfer between hardware and simulation. The abstraction also allows to exchange the currently Webots-based (Michel, 2004) simulation back end. Here we chose Webots software as our multi-body simulation software for Oncilla robot. Since the lowest API level 0 is implemented for the simulation and the hardware back end, applications implemented against any of the API level 0-2 can be switched transparently between simulation and hardware (Figure 5). By providing a common abstracted interface for both simulation
and hardware, it enables fast and easy transfer of experiments between these two domains. It is also possible to replay real experiment recordings (e.g., joint angles) in simulation, and vice-versa.

\subsection{Local and Remote Interface}
The Oncilla interface is accessible through a local C++ interface (API levels 0 and 1, Figure 5) and remotely via the open source middleware for extended language and tool support (API level 2). The low-level sensors and actuators are locally accessible through a C++ interface, using multiple inheritance to expose the node taxonomy. The local interface enables lightweight applications with fast sensor feedback running on the embedded PC without dealing with network latency. The Oncilla interface is also remotely available by the open-source middleware Robotics Service Bus (RSB) with C++, Java, Python, and Common Lisp bindings and therefore allows applications in
all four languages (Wienke and Wrede, 2011). This enables extended tool support, e.g., external logging, monitoring and recording of experiments. It supports more complex and computationally expensive applications to run on distributed PCs and control of the robot over the network. This was successfully applied and demonstrated in experiments that were specified in domain-specific languages. The experimental source code was automatically generated, as well as machine learning applications that can not run on the embedded PC due to resource limitations (Nordmann et al., 2013).

\subsection{Webots Model of Oncilla Robot}
A simulated model of Oncilla robot was created in Webots (Michel, 2004). It is based on the mechanical properties
extracted from Oncilla robot’s computer aided design (CAD) model, i.e., weight, center of mass, inertia, link dimension, and spring constant. The motivation to use a physics engine intended for games such as Open Dynamic Engine (ODE, physics engine of Webots) is a balance between simulation speed and required simulation accuracy. Internal kinematic loops in Oncilla robot’s pantograph leg, and its asymmetric actuation can be expressed as
a constraint in the underlying Linear Complementary Problem (LCP). There is a drawback to this approach; Open Dynamic Engine favors stability over accuracy, which results in a poor constraint resolution. Likely, such a simulator is well suited for fast prototyping, but less suited for on-board, model-based control. We used the default Webots actuator model for the proximal joints (hip and shoulder). This model applies a PID controller, with a maximum output velocity and torque limited by the theoretical motor limits, 
i.e., a maximum torque of 53.5mNm ・ 84 = 4.5Nm and 
a maximum speed of 16,300 rmp /60 s ・ 2 ・ pi/84 = 20.3 rad/s 
(53.5mNm constant motor torque, overall gear ratio n = 84, 16,300 rpm no-load motor speed). 
For the leg’s flexion and extension DOF we are directly manipulating the LCP constraint to control the mechanical stop of the diagonal spring. Since there is no easy way to specify the maximum torque or linear force in ODE to satisfy a given constraint, we transformed this force constraint into a velocity constraint using a linear motor model with internal resistance. We simplified and assumed that the motor torque required for actuating the leg
length cable was caused by the compressive force of the diagonal spring. In reality, this torque is an upper bound since external forces could induce additional leg flexion. We further limited the maximum speed at which motors move to the mechanical stop constraint for the next simulation step, proportionally to the instantaneous torque. This limit is ranging from maximum speed with no torque required, to zero speed at maximum motor
torque requested. The resulting model corresponds to a simple, linear motor model. Finally an implementation of the C++ interface level 0 back end was developed. It provides the user with the ability to use the same API to seamlessly switch control between either the real hardware or the simulated robot.

